Cultural Compass: Predicting Transfer Learning Success in Offensive Language Detection with Cultural Features

The increasing ubiquity of language technology necessitates a shift towards considering cultural diversity in the machine learning realm, particularly for subjective tasks that rely heavily on cultural nuances, such as Offensive Language Detection (OLD). Current understanding underscores that these tasks are substantially influenced by cultural values, however, a notable gap exists in determining if cultural features can accurately predict the success of cross-cultural transfer learning for such subjective tasks. Addressing this, our study delves into the intersection of cultural features and transfer learning effectiveness. The findings reveal that cultural value surveys indeed possess a predictive power for cross-cultural transfer learning success in OLD tasks and that it can be further improved using offensive word distance. Based on these results, we advocate for the integration of cultural information into datasets. Additionally, we recommend leveraging data sources rich in cultural information, such as surveys, to enhance cultural adaptability. Our research signifies a step forward in the quest for more inclusive, culturally sensitive language technologies.

==> Table/group_result.tex <==
% new
% \begin{table*}[t]
% \centering
% \scalebox{0.85}{
% \begin{tabular}{lrrrrrrrr}
% \toprule
% \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{2}{c|}{\textbf{Data-specific}}                & \multicolumn{2}{c|}{\textbf{Typology}}                     & \multicolumn{2}{c|}{\textbf{Geography}}                    & \multicolumn{2}{c}{\textbf{Orthography}}    \\
% \multicolumn{1}{l|}{}                                   & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \textbf{NDCG}        \\ \midrule
% \multicolumn{1}{l|}{\textbf{COLD}}                      & 75.00                & \multicolumn{1}{r|}{69.58}          & 25.00                & \multicolumn{1}{r|}{15.79}          & 26.67                & \multicolumn{1}{r|}{38.21}          & 58.33                & 82.07                \\
% \multicolumn{1}{l|}{\textbf{ChileOLD}}                  & 39.29                & \multicolumn{1}{r|}{60.83}          & 20.83                & \multicolumn{1}{r|}{-3.31}          & 29.17                & \multicolumn{1}{r|}{57.31}          & 29.17                & 28.07                \\
% \multicolumn{1}{l|}{\textbf{DeTox}}                     & 22.62                & \multicolumn{1}{r|}{31.47}          & 26.79                & \multicolumn{1}{r|}{47.53}          & 24.29                & \multicolumn{1}{r|}{35.38}          & 33.33                & 59.26                \\
% \multicolumn{1}{l|}{\textbf{Hindi}}                     & 83.33                & \multicolumn{1}{r|}{94.34}          & 25.00                & \multicolumn{1}{r|}{23.59}          & 25.00                & \multicolumn{1}{r|}{38.21}          & 41.67                & 77.00                \\
% \multicolumn{1}{l|}{\textbf{KOLD}}                      & 64.29                & \multicolumn{1}{r|}{79.72}          & 32.5                 & \multicolumn{1}{r|}{21.24}          & 26.67                & \multicolumn{1}{r|}{38.21}          & 37.50                & 67.45                \\
% \multicolumn{1}{l|}{\textbf{NJH\_UK}}                   & 41.67                & \multicolumn{1}{r|}{48.35}          & 64.29                & \multicolumn{1}{r|}{69.58}          & 29.17                & \multicolumn{1}{r|}{76.41}          & 45.00                & 70.28                \\
% \multicolumn{1}{l|}{\textbf{NJH\_US}}                   & 36.67                & \multicolumn{1}{r|}{79.72}          & 62.5                 & \multicolumn{1}{r|}{71.93}          & 29.17                & \multicolumn{1}{r|}{63.68}          & 33.33                & 54.59                \\
% \multicolumn{1}{l|}{\textbf{PolEval}}                   & 32.06                & \multicolumn{1}{r|}{42.38}          & 33.13                & \multicolumn{1}{r|}{29.12}          & 45.24                & \multicolumn{1}{r|}{51.13}          & 63.89                & 55.82                \\
% \multicolumn{1}{l|}{\textbf{TurkishOLD}}                & 26.79                & \multicolumn{1}{r|}{52.83}          & 70.00                & \multicolumn{1}{r|}{67.24}          & 40.00                & \multicolumn{1}{r|}{53.49}          & 24.29                & 24.17                \\ \midrule
% \multicolumn{1}{l|}{\textbf{AVG.}}                      & \textbf{46.86}       & \multicolumn{1}{r|}{\textbf{62.14}} & \textbf{40.00}       & \multicolumn{1}{r|}{\textbf{38.08}} & \textbf{30.6}        & \multicolumn{1}{r|}{\textbf{50.23}} & \textbf{40.72}       & \textbf{57.63}       \\ \midrule \midrule
%                                                         % & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule
% \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{2}{c|}{\textbf{Pragmatic}}                    & \multicolumn{2}{c|}{\textbf{PRAG}}                         & \multicolumn{2}{c|}{\textbf{OFF}}                          & \multicolumn{2}{c}{\textbf{Cultural}}       \\
% \multicolumn{1}{l|}{}                                   & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \textbf{NDCG}        \\ \midrule
% \multicolumn{1}{l|}{\textbf{COLD}}                      & 33.33                & \multicolumn{1}{r|}{65.10}          & 45.00                & \multicolumn{1}{r|}{79.24}          & 24.29                & \multicolumn{1}{r|}{9.55}          & 58.33                & 73.11                \\
% \multicolumn{1}{l|}{\textbf{ChileOLD}}                  & 26.79                & \multicolumn{1}{r|}{31.59}          & 26.79                & \multicolumn{1}{r|}{31.38}          & 26.79                & \multicolumn{1}{r|}{15.10}          & 45.00                & 78.76                \\
% \multicolumn{1}{l|}{\textbf{DeTox}}                     & 26.67                & \multicolumn{1}{r|}{27.37}          & 26.67                & \multicolumn{1}{r|}{22.11}          & 66.67                & \multicolumn{1}{r|}{77.78}          & 62.5                 & 76.35                \\
% \multicolumn{1}{l|}{\textbf{Hindi}}                     & 62.50                & \multicolumn{1}{r|}{68.41}          & 41.67                & \multicolumn{1}{r|}{56.35}          & 20.83                & \multicolumn{1}{r|}{35.02}          & 30.95                & 42.69                \\
% \multicolumn{1}{l|}{\textbf{KOLD}}                      & 41.67                & \multicolumn{1}{r|}{42.69}          & 50.00                & \multicolumn{1}{r|}{55.18}          & 66.67                & \multicolumn{1}{r|}{79.72}          & 30.95                & 23.59                \\
% \multicolumn{1}{l|}{\textbf{NJH\_UK}}                   & 83.33                & \multicolumn{1}{r|}{94.34}          & 100.00               & \multicolumn{1}{r|}{96.69}          & 62.50                & \multicolumn{1}{r|}{80.31}          & 66.67                & 79.72                \\
% \multicolumn{1}{l|}{\textbf{NJH\_US}}                   & 75.00                & \multicolumn{1}{r|}{71.93}          & 75.00                & \multicolumn{1}{r|}{71.93}          & 66.67               & \multicolumn{1}{r|}{70.17}          & 39.29                & 59.66                \\
% \multicolumn{1}{l|}{\textbf{PolEval}}                   & 68.06                & \multicolumn{1}{r|}{71.51}          & 56.94                & \multicolumn{1}{r|}{63.98}          & 45.24                & \multicolumn{1}{r|}{54.26}          & 100.00               & 99.01                \\
% \multicolumn{1}{l|}{\textbf{TurkishOLD}}                & 66.67                & \multicolumn{1}{r|}{79.72}          & 32.50                & \multicolumn{1}{r|}{65.21}          & 22.50                & \multicolumn{1}{r|}{55.66}          & 50.00                & 46.21                \\ \midrule
% \multicolumn{1}{l|}{\textbf{AVG.}}                      & \textbf{53.78}       & \multicolumn{1}{r|}{\textbf{61.41}} & \textbf{50.51}       & \multicolumn{1}{r|}{\textbf{60.23}} & \textbf{44.68}       & \multicolumn{1}{r|}{\textbf{53.06}} & \textbf{53.74}       & \textbf{64.34}       \\ \bottomrule
% \end{tabular}}
% \caption{Performance comparison of OLD ranking predictions.}
% \label{tab:new_baseline}
% \end{table*}


% old
\begin{table*}[ht]
\centering
\scalebox{0.9}{
\begin{tabular}{lrrrrrrrr}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{2}{c|}{\textbf{Data-specific}}                & \multicolumn{2}{c|}{\textbf{Typology}}                     & \multicolumn{2}{c|}{\textbf{Geography}}                    & \multicolumn{2}{c}{\textbf{Orthography}}    \\
\multicolumn{1}{l|}{}                                   & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \textbf{NDCG}        \\ \midrule
\multicolumn{1}{l|}{\textbf{COLD}}                      & 75.00                & \multicolumn{1}{r|}{69.58}          & 25.00                & \multicolumn{1}{r|}{15.79}          & 26.67                & \multicolumn{1}{r|}{38.21}          & 58.33                & 82.07                \\
\multicolumn{1}{l|}{\textbf{ChileOLD}}                  & 39.29                & \multicolumn{1}{r|}{60.83}          & 20.83                & \multicolumn{1}{r|}{-3.31}          & 29.17                & \multicolumn{1}{r|}{57.31}          & 29.17                & 28.07                \\
\multicolumn{1}{l|}{\textbf{DeTox}}                     & 22.62                & \multicolumn{1}{r|}{31.47}          & 26.79                & \multicolumn{1}{r|}{47.53}          & 24.29                & \multicolumn{1}{r|}{35.38}          & 33.33                & 59.26                \\
\multicolumn{1}{l|}{\textbf{Hindi}}                     & 83.33                & \multicolumn{1}{r|}{94.34}          & 25.00                & \multicolumn{1}{r|}{23.59}          & 25.00                & \multicolumn{1}{r|}{38.21}          & 41.67                & 77.00                \\
\multicolumn{1}{l|}{\textbf{KOLD}}                      & 64.29                & \multicolumn{1}{r|}{79.72}          & 32.5                 & \multicolumn{1}{r|}{21.24}          & 26.67                & \multicolumn{1}{r|}{38.21}          & 37.50                & 67.45                \\
\multicolumn{1}{l|}{\textbf{NJH\_UK}}                   & 41.67                & \multicolumn{1}{r|}{48.35}          & 64.29                & \multicolumn{1}{r|}{69.58}          & 29.17                & \multicolumn{1}{r|}{76.41}          & 45.00                & 70.28                \\
\multicolumn{1}{l|}{\textbf{NJH\_US}}                   & 36.67                & \multicolumn{1}{r|}{79.72}          & 62.5                 & \multicolumn{1}{r|}{71.93}          & 29.17                & \multicolumn{1}{r|}{63.68}          & 33.33                & 54.59                \\
\multicolumn{1}{l|}{\textbf{PolEval}}                   & 32.06                & \multicolumn{1}{r|}{42.38}          & 33.13                & \multicolumn{1}{r|}{29.12}          & 45.24                & \multicolumn{1}{r|}{51.13}          & 63.89                & 55.82                \\
\multicolumn{1}{l|}{\textbf{TurkishOLD}}                & 26.79                & \multicolumn{1}{r|}{52.83}          & 70.00                & \multicolumn{1}{r|}{67.24}          & 40.00                & \multicolumn{1}{r|}{53.49}          & 24.29                & 24.17                \\ \midrule
\multicolumn{1}{l|}{\textbf{AVG.}}                      & \textbf{46.86}       & \multicolumn{1}{r|}{\textbf{62.14}} & \textbf{40.00}       & \multicolumn{1}{r|}{\textbf{38.08}} & \textbf{30.6}        & \multicolumn{1}{r|}{\textbf{50.23}} & \textbf{40.72}       & \textbf{57.63}       \\ \midrule
 \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{2}{c|}{\textbf{Pragmatic}}                    & \multicolumn{2}{c|}{\textbf{PRAG}}                         & \multicolumn{2}{c|}{\textbf{OFF}}                          & \multicolumn{2}{c}{\textbf{Cultural}}       \\
\multicolumn{1}{l|}{}                                   & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \multicolumn{1}{r|}{\textbf{NDCG}}  & \textbf{MAP}         & \textbf{NDCG}        \\ \midrule
\multicolumn{1}{l|}{\textbf{COLD}}                      & 33.33                & \multicolumn{1}{r|}{65.10}          & 45.00                & \multicolumn{1}{r|}{79.24}          & 25.00                & \multicolumn{1}{r|}{47.76}          & 58.33                & 73.11                \\
\multicolumn{1}{l|}{\textbf{ChileOLD}}                  & 26.79                & \multicolumn{1}{r|}{31.59}          & 26.79                & \multicolumn{1}{r|}{31.38}          & 29.17                & \multicolumn{1}{r|}{42.69}          & 45.00                & 78.76                \\
\multicolumn{1}{l|}{\textbf{DeTox}}                     & 26.67                & \multicolumn{1}{r|}{27.37}          & 26.67                & \multicolumn{1}{r|}{22.11}          & 83.33                & \multicolumn{1}{r|}{73.28}          & 62.5                 & 76.35                \\
\multicolumn{1}{l|}{\textbf{Hindi}}                     & 62.50                & \multicolumn{1}{r|}{68.41}          & 41.67                & \multicolumn{1}{r|}{56.35}          & 29.17                & \multicolumn{1}{r|}{39.38}          & 30.95                & 42.69                \\
\multicolumn{1}{l|}{\textbf{KOLD}}                      & 41.67                & \multicolumn{1}{r|}{42.69}          & 50.00                & \multicolumn{1}{r|}{55.18}          & 83.33                & \multicolumn{1}{r|}{85.38}          & 30.95                & 23.59                \\
\multicolumn{1}{l|}{\textbf{NJH\_UK}}                   & 83.33                & \multicolumn{1}{r|}{94.34}          & 100.00               & \multicolumn{1}{r|}{96.69}          & 75.00                & \multicolumn{1}{r|}{80.31}          & 66.67                & 79.72                \\
\multicolumn{1}{l|}{\textbf{NJH\_US}}                   & 75.00                & \multicolumn{1}{r|}{71.93}          & 75.00                & \multicolumn{1}{r|}{71.93}          & 100.00               & \multicolumn{1}{r|}{93.28}          & 39.29                & 59.66                \\
\multicolumn{1}{l|}{\textbf{PolEval}}                   & 68.06                & \multicolumn{1}{r|}{71.51}          & 56.94                & \multicolumn{1}{r|}{63.98}          & 64.29                & \multicolumn{1}{r|}{40.41}          & 100.00               & 99.01                \\
\multicolumn{1}{l|}{\textbf{TurkishOLD}}                & 66.67                & \multicolumn{1}{r|}{79.72}          & 32.50                & \multicolumn{1}{r|}{65.21}          & 25.00                & \multicolumn{1}{r|}{42.10}          & 50.00                & 46.21                \\ \midrule
\multicolumn{1}{l|}{\textbf{AVG.}}                      & \textbf{53.78}       & \multicolumn{1}{r|}{\textbf{61.41}} & \textbf{50.51}       & \multicolumn{1}{r|}{\textbf{60.23}} & \textbf{57.14}       & \multicolumn{1}{r|}{\textbf{60.51}} & \textbf{53.74}       & \textbf{64.34}       \\ \bottomrule
\end{tabular}}
\caption{Performance comparison of OLD ranking predictions.}
\label{tab:new_baseline}
\end{table*}
